Triangulating an exotic T quark

Limits on an exotic heavy quark $T$ are broadly generalized by considering the full range of $T\rightarrow Wb, th$ or $tZ$ branching ratios. We combine results of specific $T\rightarrow tZ$ and $T\rightarrow Wb$ searches with limits on various combinations of decay modes evaluated by re-interpreting other searches. We find strong bounds across the entire space of branching ratios, ranging from $m_T > 415$ GeV to $m_T > 557$ GeV at 95% confidence level.

==> table_Wb.tex <==
\begin{table} 
 \caption{ Details of the predicted limit on $T$ pair-production and 
  $T\rightarrow Wb$ decays,  using basis templates from $b'\rightarrow 
  Wt$ decays at ATLAS.} 
 \label{tab:Wb}
\begin{tabular}{lrrrrrrr}
\hline\hline 
 &$T_{300}$ & $T_{350}$ & $T_{400}$ & $T_{450}$ & $T_{500}$ & $T_{550}$ & $T_{600}$ \\ \hline

 $a_{b' 300}$  & 0.23  & 0.09  & 0.03  & 0.01  & 0.01  & 2e-3  & 1e-3  \\
 $a_{b' 300}$  & 0  & 0  & 0  & 0  & 0  & 0  & 0  \\
 $a_{b' 300}$  & 0  & 0  & 0  & 0  & 0  & 0  & 0  \\
 $a_{b' 300}$  & 0  & 0  & 0  & 0  & 0  & 0  & 0  \\
 $a_{b' 300}$  & 0  & 0  & 0  & 1e-3  & 0  & 0  & 0  \\
 $a_{b' 300}$  & 0.01  & 0.06  & 0.01  & 0.03  & 0.01  & 0  & 3e-3  \\
 $a_{b' 300}$  & 7.72  & 4.21  & 3.03  & 1.5  & 0.73  & 0.37  & 0.20  \\\hline 
$\sigma^{\rm limit}_i/\sigma_i^{\rm theory}$ (pred) & 0.31  & 0.66  & 1.16  & 2.36  & 4.83  & 9.81  & 17.85  \\
$\sigma^{\rm limit}$ [pb] (pred) & 2.5  & 2.12  & 1.64  & 1.57  & 1.6  & 1.68  & 1.65  \\ 
 \hline\hline 
 \end{tabular} 
 \end{table}


==> table_tZWb.tex <==
\begin{table} 
 \caption{ Details of the predicted limit on $T$ pair-production with 
  $T\rightarrow tZ,Wb$ decays,  using basis templates from $b'\rightarrow 
  Wt$ decays at ATLAS.} 
 \label{tab:tZWb}
\begin{tabular}{lrrrrrrr}
\hline\hline 
 &$T_{300}$ & $T_{350}$ & $T_{400}$ & $T_{450}$ & $T_{500}$ & $T_{550}$ & $T_{600}$ \\ \hline

 $a_{b' 300}$  & 0.305  & 0.109  & 0.031  & 0.011  & 0.003  & 0.001  & 0  \\
 $a_{b' 300}$  & 0  & 0  & 0  & 0  & 0  & 0  & 0  \\
 $a_{b' 300}$  & 0  & 0  & 0  & 0  & 0  & 0  & 0  \\
 $a_{b' 300}$  & 0  & 0  & 0  & 0  & 0  & 0  & 0  \\
 $a_{b' 300}$  & 0.017  & 0.019  & 0.013  & 0.001  & 0.004  & 0  & 0  \\
 $a_{b' 300}$  & 0.059  & 0.105  & 0.042  & 0.024  & 0.01  & 0.034  & 0.002  \\
 $a_{b' 300}$  & 5.49  & 4.711  & 3.973  & 2.318  & 1.318  & 0.636  & 0.394  \\\hline 
$\sigma^{\rm limit}_i/\sigma_i^{\rm theory}$ (pred) & 0.31  & 0.55  & 0.88  & 1.62  & 3.02  & 5.84  & 10.5  \\
$\sigma^{\rm limit}$ [pb] (pred) & 2.53  & 1.77  & 1.24  & 1.07  & 1  & 1  & 0.97  \\ 
 \hline\hline 
 \end{tabular} 
 \end{table}

